Solving Dynamic Discrete Choice Models Using Smoothing and Sieve Methods

We propose to combine smoothing, simulations and sieve approximations to solve for either the integrated or expected value function in a general class of dynamic discrete choice (DDC) models. We use importance sampling to approximate the Bellman operators defining the two functions. The random Bellman operators, and therefore also the corresponding solutions, are generally non-smooth which is undesirable. To circumvent this issue, we introduce a smoothed version of the random Bellman operator and solve for the corresponding smoothed value function using sieve methods. We show that one can avoid using sieves by generalizing and adapting the `self-approximating' method of Rust (1997) to our setting. We provide an asymptotic theory for the approximate solutions and show that they converge with root-N-rate, where $N$ is number of Monte Carlo draws, towards Gaussian processes. We examine their performance in practice through a set of numerical experiments and find that both methods perform well with the sieve method being particularly attractive in terms of computational speed and accuracy.

==> fig/README <==
In .tex figures add

\tikzstyle{every node}=[font=\small]

height = {55.0mm}

\hspace{0.4cm}

fjern "axis lines* = left"

sæt samme ticks

width = {70.0mm}, legend style={font=\small},


==> figs_rev1/contractionorquality.tex <==
\begin{tikzpicture}[]
\begin{axis}[height = {50.0mm}, legend pos = {north east}, legend style={nodes={scale=0.6, transform shape}}, ylabel = {$v(z)$}, xmin = {0.0}, xmax = {1000.0}, ymax = {0}, xlabel = {Mileage, $z$}, {unbounded coords=jump, scaled x ticks = false, xticklabel style={rotate = 0}, xmajorgrids = true, xtick = {0.0,200.0,400.0,600.0,800.0,1000.0}, xticklabels = {0,200,400,600,800,1000}, xtick align = inside, axis lines* = left, scaled y ticks = false, yticklabel style={rotate = 0}, ymajorgrids = true, ytick = {-20.0,-15.0,-10.0,-5.0,0.0}, yticklabels = {-20,-15,-10,-5,0}, ytick align = inside, axis lines* = left,     xshift = 0.0mm,
    yshift = 0.0mm,
    axis background/.style={fill={rgb,1:red,1.00000000;green,1.00000000;blue,1.00000000}}
}, ymin = {-24}, width = {90.0mm}]\addplot+ [color = {rgb,1:red,0.50196078;green,0.50196078;blue,0.50196078},
draw opacity=1.0,
line width=3,
solid,mark = none,
mark size = 2.0,
mark options = {
    color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000}, draw opacity = 1.0,
    fill = {rgb,1:red,0.50196078;green,0.50196078;blue,0.50196078}, fill opacity = 1.0,
    line width = 1,
    rotate = 0,
    solid
}]coordinates {
(0.0, -3.037228169189243)
(1.0069334586852996, -3.074870458653453)
(3.0187725460755765, -3.1499851003081134)
(6.031465685989557, -3.262227865113735)
(10.038945715380665, -3.4110712669271646)
(15.033142102795605, -3.595790470990419)
(21.003997201350987, -3.8154432957960203)
(27.93948650349537, -4.068843289030532)
(35.825642856767374, -4.3545246463861975)
(44.64658459178189, -4.670697718017638)
(54.38454750579885, -5.015194065168148)
(65.01992063746303, -5.385400947180762)
(76.5312857606707, -5.7781870035013565)
(88.8954605180265, -6.189824680818187)
(102.087545107026, -6.615921077751892)
(116.08097242494414, -7.051378061095572)
(130.84756157144483, -7.490413241235015)
(146.35757460116355, -7.926681962390017)
(162.57977641197175, -8.353537789118992)
(179.4814976483156, -8.764444703737588)
(197.02870049295075, -9.153502819959332)
(215.186047214576, -9.515985711552606)
(233.9169713333214, -9.848747494279525)
(253.18375126077242, -10.150380277019288)
(272.9475862662288, -10.42108750467587)
(293.16867461621297, -10.662339589700828)
(313.80629372986334, -10.876435391086574)
(334.81888218879385, -11.066086763842375)
(356.16412343625865, -11.234095619266114)
(377.7990309970662, -11.383142132017856)
(399.68003504661937, -11.515669224119858)
(421.7630701547439, -11.63383646934425)
(444.0036640276005, -11.73951694504845)
(466.3570270689659, -11.834317352962351)
(488.7781425805191, -11.919608066099403)
(511.2218574194808, -11.9965557097353)
(533.642972931034, -12.066154016649591)
(555.9963359723994, -12.129251463472666)
(578.236929845256, -12.186574898590528)
(600.3199649533806, -12.238749542416496)
(622.2009690029338, -12.286315479739457)
(643.8358765637414, -12.329741391774544)
(665.181117811206, -12.369435730475665)
(686.1937062701364, -12.40575603157453)
(706.8313253837871, -12.439016458160761)
(727.052413733771, -12.469494154927464)
(746.8162487392276, -12.497434381576259)
(766.0830286666785, -12.523054914279374)
(784.8139527854239, -12.546549583397553)
(802.9712995070491, -12.568091383718748)
(820.5185023516843, -12.587834944689426)
(837.4202235880283, -12.605918779261224)
(853.6424253988364, -12.62246702632045)
(869.1524384285551, -12.637591118901014)
(883.9190275750559, -12.65139101673024)
(897.912454892974, -12.663956480531759)
(911.1045394819735, -12.675367933399915)
(923.4687142393292, -12.685697469563504)
(934.9800793625369, -12.6950094303103)
(945.6154524942011, -12.703361239728373)
(955.3534154082181, -12.710803739959275)
(964.1743571432327, -12.717381880400616)
(972.0605134965045, -12.723134559507248)
(978.9960027986491, -12.728093816101918)
(984.9668578972044, -12.732279714480704)
(989.9610542846193, -12.735690999798734)
(993.9685343140103, -12.738293401688452)
(996.9812274539245, -12.740075631826535)
(998.9930665413146, -12.741157514976987)
(1000.0, -12.741675728967731)
};
\addlegendentry{limit solution}
\addplot+ [color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000},
draw opacity=1.0,
line width=1,
dotted,mark = none,
mark size = 2.0,
mark options = {
    color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000}, draw opacity = 1.0,
    fill = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000}, fill opacity = 1.0,
    line width = 1,
    rotate = 0,
    solid
}]coordinates {
(0.0, -18.996985943294742)
(1.0069334586852996, -18.99899971869473)
(3.0187725460755765, -19.003023213466165)
(6.031465685989557, -19.009048323719156)
(10.038945715380665, -19.017062914020467)
(15.033142102795605, -19.027050841829453)
(21.003997201350987, -19.03899199000293)
(27.93948650349537, -19.05286230730353)
(35.825642856767374, -19.068633856830235)
(44.64658459178189, -19.08627487227366)
(54.38454750579885, -19.105749821883133)
(65.01992063746303, -19.127019480016973)
(76.5312857606707, -19.15004100613225)
(88.8954605180265, -19.17476803105524)
(102.087545107026, -19.20115075035945)
(116.08097242494414, -19.229136024663397)
(130.84756157144483, -19.258667486646885)
(146.35757460116355, -19.28968565457076)
(162.57977641197175, -19.322128052072163)
(179.4814976483156, -19.355929333994705)
(197.02870049295075, -19.391021418000946)
(215.186047214576, -19.427333621702818)
(233.9169713333214, -19.464792805034644)
(253.18375126077242, -19.5033235175829)
(272.9475862662288, -19.542848150576745)
(293.16867461621297, -19.583287093234144)
(313.80629372986334, -19.624558893149366)
(334.81888218879385, -19.666580420399722)
(356.16412343625865, -19.709267035041535)
(377.7990309970662, -19.752532757658667)
(399.68003504661937, -19.79629044262042)
(421.7630701547439, -19.840451953700075)
(444.0036640276005, -19.884928341700384)
(466.3570270689659, -19.929630023727928)
(488.7781425805191, -19.97446696375473)
(511.2218574194808, -20.01934885410245)
(533.642972931034, -20.064185297482442)
(555.9963359723994, -20.10888598922316)
(578.236929845256, -20.15336089931595)
(600.3199649533806, -20.19752045390979)
(622.2009690029338, -20.241275715886616)
(643.8358765637414, -20.28453856414999)
(665.181117811206, -20.327221871262257)
(686.1937062701364, -20.369239679068283)
(706.8313253837871, -20.41050737194763)
(727.052413733771, -20.450941847341696)
(746.8162487392276, -20.49046168320767)
(766.0830286666785, -20.528987302057562)
(784.8139527854239, -20.56644113124745)
(802.9712995070491, -20.60274775919021)
(820.5185023516843, -20.637834087173548)
(837.4202235880283, -20.67162947647485)
(853.6424253988364, -20.70406589047449)
(869.1524384285551, -20.73507803148056)
(883.9190275750559, -20.7646034719895)
(897.912454892974, -20.79258278011974)
(911.1045394819735, -20.818959638968376)
(923.4687142393292, -20.843680959654552)
(934.9800793625369, -20.866696987827208)
(945.6154524942011, -20.887961403429255)
(955.3534154082181, -20.90743141352507)
(964.1743571432327, -20.925067838012975)
(972.0605134965045, -20.94083518805967)
(978.9960027986491, -20.95470173710862)
(984.9668578972044, -20.966639584329734)
(989.9610542846193, -20.976624710392684)
(993.9685343140103, -20.98463702546147)
(996.9812274539245, -20.990660409322683)
(998.9930665413146, -20.994682743574874)
(1000.0, -20.996695935821062)
};
\addlegendentry{$v$,  K=1, L = 1.0 }
\addplot+ [color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000},
draw opacity=1.0,
line width=1,
dashed,mark = none,
mark size = 2.0,
mark options = {
    color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000}, draw opacity = 1.0,
    fill = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000}, fill opacity = 1.0,
    line width = 1,
    rotate = 0,
    solid
}]coordinates {
(0.0, -18.205347488862394)
(1.0069334586852996, -18.209274124067313)
(3.0187725460755765, -18.217119483279756)
(6.031465685989557, -18.2288677600099)
(10.038945715380665, -18.2444952842533)
(15.033142102795605, -18.263970570077337)
(21.003997201350987, -18.287254378920125)
(27.93948650349537, -18.31429979847407)
(35.825642856767374, -18.345052336994808)
(44.64658459178189, -18.37945003284512)
(54.38454750579885, -18.41742357905291)
(65.01992063746303, -18.458896462632012)
(76.5312857606707, -18.503785118385316)
(88.8954605180265, -18.551999096880376)
(102.087545107026, -18.603441246260047)
(116.08097242494414, -18.658007907522617)
(130.84756157144483, -18.715589122880253)
(146.35757460116355, -18.776068856778192)
(162.57977641197175, -18.839325229133355)
(179.4814976483156, -18.905230760327033)
(197.02870049295075, -18.97365262746472)
(215.186047214576, -19.044452931394584)
(233.9169713333214, -19.117488973956863)
(253.18375126077242, -19.19261354491795)
(272.9475862662288, -19.26967521802606)
(293.16867461621297, -19.348518655609897)
(313.80629372986334, -19.42898492112754)
(334.81888218879385, -19.510911799060196)
(356.16412343625865, -19.59413412153393)
(377.7990309970662, -19.678484101042436)
(399.68003504661937, -19.76379166863473)
(421.7630701547439, -19.849884816923687)
(444.0036640276005, -19.936589947263695)
(466.3570270689659, -20.023732220438955)
(488.7781425805191, -20.11113591019693)
(511.2218574194808, -20.198624758954487)
(533.642972931034, -20.286022334996893)
(555.9963359723994, -20.373152390480904)
(578.236929845256, -20.459839219544108)
(600.3199649533806, -20.545908015810973)
(622.2009690029338, -20.631185228573404)
(643.8358765637414, -20.715498916909002)
(665.181117811206, -20.798679100983698)
(686.1937062701364, -20.880558109767893)
(706.8313253837871, -20.960970924376852)
(727.052413733771, -21.03975551622727)
(746.8162487392276, -21.116753179185046)
(766.0830286666785, -21.191808854863922)
(784.8139527854239, -21.26477145022435)
(802.9712995070491, -21.335494146616497)
(820.5185023516843, -21.403834699414773)
(837.4202235880283, -21.46965572740349)
(853.6424253988364, -21.532824991097364)
(869.1524384285551, -21.59321565921772)
(883.9190275750559, -21.65070656259586)
(897.912454892974, -21.705182434840204)
(911.1045394819735, -21.756534139182683)
(923.4687142393292, -21.80465888101151)
(934.9800793625369, -21.849460405699233)
(945.6154524942011, -21.890849181444647)
(955.3534154082181, -21.928742566960096)
(964.1743571432327, -21.963064963948092)
(972.0605134965045, -21.993747954418005)
(978.9960027986491, -22.020730422989562)
(984.9668578972044, -22.043958664411562)
(989.9610542846193, -22.06338647658534)
(993.9685343140103, -22.078975239422917)
(996.9812274539245, -22.09069397988442)
(998.9930665413146, -22.098519423530018)
(1000.0, -22.102436032888303)
};
\addlegendentry{$V$, K=1, L = 1.0 }
\addplot+ [color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000},
draw opacity=1.0,
line width=2,
dotted,mark = none,
mark size = 2.0,
mark options = {
    color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000}, draw opacity = 1.0,
    fill = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000}, fill opacity = 1.0,
    line width = 1,
    rotate = 0,
    solid
}]coordinates {
(0.0, -3.1211726949092258)
(1.0069334586852996, -3.158607915818727)
(3.0187725460755765, -3.233117346553291)
(6.031465685989557, -3.343983881438089)
(10.038945715380665, -3.49014406905395)
(15.033142102795605, -3.6702025254295547)
(21.003997201350987, -3.8824507600824205)
(27.93948650349537, -4.124890080018513)
(35.825642856767374, -4.395258152711902)
(44.64658459178189, -4.6910587229048435)
(54.38454750579885, -5.009593887919897)
(65.01992063746303, -5.347998240234071)
(76.5312857606707, -5.703274083851631)
(88.8954605180265, -6.072326825900127)
(102.087545107026, -6.451999548308796)
(116.08097242494414, -6.839105702044879)
(130.84756157144483, -7.230458885368186)
(146.35757460116355, -7.622898842750901)
(162.57977641197175, -8.013313254287876)
(179.4814976483156, -8.398655688465205)
(197.02870049295075, -8.775961340440105)
(215.186047214576, -9.1423638294733)
(233.9169713333214, -9.495118097995562)
(253.18375126077242, -9.831635700396772)
(272.9475862662288, -10.149538488747108)
(293.16867461621297, -10.446733788767453)
(313.80629372986334, -10.721508046769056)
(334.81888218879385, -10.97262748229643)
(356.16412343625865, -11.199426336444363)
(377.7990309970662, -11.401859983097618)
(399.68003504661937, -11.580504670199822)
(421.7630701547439, -11.736497698878933)
(444.0036640276005, -11.871426963485769)
(466.3570270689659, -11.987190627027324)
(488.7781425805191, -12.085851873957662)
(511.2218574194808, -12.169509933974)
(533.642972931034, -12.240200125654844)
(555.9963359723994, -12.299826645395955)
(578.236929845256, -12.350125072674434)
(600.3199649533806, -12.392647996023982)
(622.2009690029338, -12.428766305012362)
(643.8358765637414, -12.459679520998565)
(665.181117811206, -12.48643010376089)
(686.1937062701364, -12.509918337149776)
(706.8313253837871, -12.530915840883829)
(727.052413733771, -12.550076866465666)
(746.8162487392276, -12.56794731457625)
(766.0830286666785, -12.584971905172015)
(784.8139527854239, -12.601500194395916)
(802.9712995070491, -12.617792213803854)
(820.5185023516843, -12.63402444968337)
(837.4202235880283, -12.65029672102412)
(853.6424253988364, -12.666640289653266)
(869.1524384285551, -12.683027280431228)
(883.9190275750559, -12.699381237862317)
(897.912454892974, -12.7155884301984)
(911.1045394819735, -12.731509359788646)
(923.4687142393292, -12.746989866774035)
(934.9800793625369, -12.761871228117924)
(945.6154524942011, -12.775998748217907)
(955.3534154082181, -12.789228491909032)
(964.1743571432327, -12.801431998331395)
(972.0605134965045, -12.81249900498476)
(978.9960027986491, -12.822338378551802)
(984.9668578972044, -12.830877573748252)
(989.9610542846193, -12.838045976624965)
(993.9685343140103, -12.84346139830471)
(996.9812274539245, -12.846570507475072)
(998.9930665413146, -12.847905448237096)
(1000.0, -12.848405538279776)
};
\addlegendentry{$v$,  K=4, L = 1.78 }
\addplot+ [color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000},
draw opacity=1.0,
line width=2,
dashed,mark = none,
mark size = 2.0,
mark options = {
    color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000}, draw opacity = 1.0,
    fill = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000}, fill opacity = 1.0,
    line width = 1,
    rotate = 0,
    solid
}]coordinates {
(0.0, -3.1138805843718136)
(1.0069334586852996, -3.1509938722871254)
(3.0187725460755765, -3.2248770616166653)
(6.031465685989557, -3.334847980402219)
(10.038945715380665, -3.4798947880745565)
(15.033142102795605, -3.6586894367148344)
(21.003997201350987, -3.8696052170356063)
(27.93948650349537, -4.110738036939775)
(35.825642856767374, -4.379930980929598)
(44.64658459178189, -4.674801587696333)
(54.38454750579885, -4.992771155687838)
(65.01992063746303, -5.331095237062412)
(76.5312857606707, -5.686894306441378)
(88.8954605180265, -6.057183397196574)
(102.087545107026, -6.438899306384385)
(116.08097242494414, -6.828923832629834)
(130.84756157144483, -7.224101532181146)
(146.35757460116355, -7.621250830116223)
(162.57977641197175, -8.017168258877652)
(179.4814976483156, -8.408627419984784)
(197.02870049295075, -8.792377226963916)
(215.186047214576, -9.165148038611543)
(233.9169713333214, -9.523678672268705)
(253.18375126077242, -9.86478006294864)
(272.9475862662288, -10.185449297308256)
(293.16867461621297, -10.483037453577806)
(313.80629372986334, -10.755455195667333)
(334.81888218879385, -11.00137653631123)
(356.16412343625865, -11.220385563116036)
(377.7990309970662, -11.413016133986124)
(399.68003504661937, -11.580663729844293)
(421.7630701547439, -11.725389254751118)
(444.0036640276005, -11.849665657299367)
(466.3570270689659, -11.956125781139152)
(488.7781425805191, -12.047355392353946)
(511.2218574194808, -12.12575130683918)
(533.642972931034, -12.193443475268005)
(555.9963359723994, -12.25226776738222)
(578.236929845256, -12.303772685850298)
(600.3199649533806, -12.349245082566933)
(622.2009690029338, -12.38974390078445)
(643.8358765637414, -12.426134968656088)
(665.181117811206, -12.459123034391204)
(686.1937062701364, -12.48927939782252)
(706.8313253837871, -12.517064817247526)
(727.052413733771, -12.542848092042224)
(746.8162487392276, -12.566921050204188)
(766.0830286666785, -12.589510757610341)
(784.8139527854239, -12.610789712332164)
(802.9712995070491, -12.63088465619085)
(820.5185023516843, -12.6498844680331)
(837.4202235880283, -12.66784742792669)
(853.6424253988364, -12.684807980644221)
(869.1524384285551, -12.700782997217443)
(883.9190275750559, -12.715777446149062)
(897.912454892974, -12.729789345525184)
(911.1045394819735, -12.742813871069599)
(923.4687142393292, -12.754846533989511)
(934.9800793625369, -12.765885402794042)
(945.6154524942011, -12.775932410199575)
(955.3534154082181, -12.784993846410744)
(964.1743571432327, -12.793080183981559)
(972.0605134965045, -12.800205402568539)
(978.9960027986491, -12.806385984401498)
(984.9668578972044, -12.81163973702585)
(989.9610542846193, -12.815981029660957)
(993.9685343140103, -12.819345973527028)
(996.9812274539245, -12.821624960865682)
(998.9930665413146, -12.8229612309535)
(1000.0, -12.823587876792935)
};
\addlegendentry{$V$, K=4, L = 1.78 }
\end{axis}

\end{tikzpicture}

